A Path To DOT: Formalizing Fully Path-Dependent Types

The Dependent Object Types (DOT) calculus aims to formalize the Scala programming language with a focus on path-dependent types $-$ types such as $x.a_1\dots a_n.T$ that depend on the runtime value of a path $x.a_1\dots a_n$ to an object. Unfortunately, existing formulations of DOT can model only types of the form $x.A$ which depend on variables rather than general paths. This restriction makes it impossible to model nested module dependencies. Nesting small components inside larger ones is a necessary ingredient of a modular, scalable language. DOT's variable restriction thus undermines its ability to fully formalize a variety of programming-language features including Scala's module system, family polymorphism, and covariant specialization. This paper presents the pDOT calculus, which generalizes DOT to support types that depend on paths of arbitrary length, as well as singleton types to track path equality. We show that naive approaches to add paths to DOT make it inherently unsound, and present necessary conditions for such a calculus to be sound. We discuss the key changes necessary to adapt the techniques of the DOT soundness proofs so that they can be applied to pDOT. Our paper comes with a Coq-mechanized type-safety proof of pDOT. With support for paths of arbitrary length, pDOT can realize DOT's full potential for formalizing Scala-like calculi.

==> dottable.tex <==
\definecolor{verticalline}{HTML}{C0C0C0}
\definecolor{notinscala}{HTML}{C0C0C0}
\definecolor{scalafeatures}{HTML}{656565}
\definecolor{dottyfeatures}{HTML}{9B9B9B}
\definecolor{fullypdt}{HTML}{343434}
\definecolor{dotfeatures}{HTML}{000000}

\begin{table}[]\tiny
	\begin{tabular}{llllrl
				!{\color{verticalline}\vrule}l
				!{\color{verticalline}\vrule}l
				!{\color{verticalline}\vrule}l
				!{\color{verticalline}\vrule}l
%				!{\color{verticalline}\vrule}l
%				!{\color{verticalline}\vrule}l
%				!{\color{verticalline}\vrule}l
%				!{\color{verticalline}\vrule}l
%				!{\color{verticalline}\vrule}l
%				!{\color{verticalline}\vrule}l
			}
		\multicolumn{5}{l}{\multirow{-2}{*}{}}
		&\parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{$\nu$Obj \\ \citet{nuobj}\vspace{7mm}}}}
		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{Featherweight Scala \\ \citet{featherweight}\vspace{7mm}}}}
		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{Scalina \\ \citet{scalina}\vspace{8mm}}}}
		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{DOT \\ \citet{fool12}\vspace{8.5mm}}}}
		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{$\mu$DOT \\ \citet{oopsla14}\vspace{8.5mm}}}}
%		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{DOT \\ \citet{arxiv1}\vspace{2.5mm}}}}
%		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{DOT \\ \citet{wadlerfest}\vspace{8mm}}}}
%		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{DOT \\ \citet{oopsla16}}}}
%		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{Mutable DOT \\ \citet{mutation}}}}
%		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{$\kappa$DOT \\ \citet{constructors}\vspace{2.5mm}}}}
%		& \parbox[b]{3mm}{\rotatebox[origin=b]{90}{\makecell[l]{\textit{DOT with paths} \\ \textit{(this work)}\vspace{9.5mm}}}}
		\\
		
		\multicolumn{4}{c}{\cellcolor{notinscala} features} &
		\cellcolor{notinscala}1st class classes& 
		\cellcolor{notinscala} &&&&
%		&&&&&&
		\\
		
		 \multicolumn{4}{c}{\multirow{-2}{*}{\cellcolor{notinscala}}\textit{not} in Scala or dotty} & 
		 \cellcolor{notinscala}subtyping btw rec types& & & & & 
		 \cellcolor{notinscala} 
%		 & 
%		 \cellcolor{notinscala}
		 % & & & & & 
		 \\ %\hline

		\cellcolor{dottyfeatures} & \multicolumn{3}{l}{\cellcolor{dottyfeatures}} & 
		\cellcolor{dottyfeatures}union types &
		\cellcolor{dottyfeatures} & & & 
		\cellcolor{dottyfeatures} & 
%		& 
%		\cellcolor{dottyfeatures}
%		 & & 
%		\cellcolor{dottyfeatures} & & &
		 \\ %\hhline{>{\arrayrulecolor{notinscala}}-|>{\arrayrulecolor{black}}-|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
		
		\cellcolor{dottyfeatures} & 
		\cellcolor{scalafeatures} & 
		\multicolumn{2}{l}{\cellcolor{scalafeatures}} & 
		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} higher-kinded types} & & & 
		\cellcolor{scalafeatures} & & 
%		& & & & & &
		\\
		
%		\cellcolor{dottyfeatures}& 
%		\cellcolor{scalafeatures}& 
%		\multicolumn{2}{l}{\cellcolor{scalafeatures}}& 
%		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} mutation}&&&&&
%%		&&&&
%%		\cellcolor{scalafeatures} & 
%%		\cellcolor{scalafeatures} &
%		\\
		
		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}&
		\multicolumn{2}{l}{\cellcolor{scalafeatures}}& 
		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} inner classes}& 
		\cellcolor{scalafeatures} &
		\cellcolor{scalafeatures} &&&
%		&&&&&&
		\\

%		\cellcolor{dottyfeatures} & 
%		\cellcolor{scalafeatures} &
%		\multicolumn{2}{l}{\cellcolor{scalafeatures}} & 
%		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} higher-order fun's}   & & & & & 
%%		&&
%%		\cellcolor{scalafeatures} & &
%%		\cellcolor{scalafeatures} & 
%%		\cellcolor{scalafeatures} & 
%%		\cellcolor{scalafeatures}
%		\\

		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\multicolumn{2}{l}{\cellcolor{scalafeatures}}& 
		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} classes} & 
		\cellcolor{scalafeatures} & 
		\cellcolor{scalafeatures} & 
		\cellcolor{scalafeatures} &&
%		&&&&&&
		\\
		
		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\multicolumn{2}{l}{\cellcolor{scalafeatures}}& 
		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} nominal typing} & 
		\cellcolor{scalafeatures} & 
		\cellcolor{scalafeatures} & \cellcolor{scalafeatures} &&
%		&&&&&&
		\\
		
		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\multicolumn{2}{l}{\cellcolor{scalafeatures}}& 
		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} constructors} & 
		\cellcolor{scalafeatures} && 
		\cellcolor{scalafeatures} & 
		\cellcolor{scalafeatures} &
%		&&&&&
%		\cellcolor{scalafeatures} &
		\\
		
		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\multicolumn{2}{l}{\multirow{-8}{*}{\cellcolor{scalafeatures}}}  &
		\cellcolor{scalafeatures}{\color[HTML]{FFFFFF} singleton types} & 
		\cellcolor{scalafeatures} & 
		\cellcolor{scalafeatures} & 
		\cellcolor{scalafeatures} &&
%		&&&&&&
%		\cellcolor{scalafeatures} 
		\\ %\hhline{>{\arrayrulecolor{notinscala}}-|>{\arrayrulecolor{scalafeatures}}-|>{\arrayrulecolor{black}}-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
		
		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\cellcolor{fullypdt}& 
		\cellcolor{fullypdt} & 
		\cellcolor{fullypdt}{\color[HTML]{FFFFFF} paths} & 
		\cellcolor{fullypdt} & 
		\cellcolor{fullypdt} & 
		\cellcolor{fullypdt} & 
		\cellcolor{fullypdt} &
%		&&&&&&
%		\cellcolor{fullypdt} 
		\\ %\cline{5-16} 

		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\cellcolor{fullypdt}& 
		\cellcolor{dotfeatures} & 
		\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} top}&&& 
		\cellcolor{dotfeatures} & 
		\cellcolor{dotfeatures} &
%		& 
%		\cellcolor{dotfeatures} & 
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} & 
%		\cellcolor{dotfeatures} & 
%		\cellcolor{dotfeatures} &
%		 \cellcolor{dotfeatures}
		 \\

		\cellcolor{dottyfeatures}&
		\cellcolor{scalafeatures}& 
		\cellcolor{fullypdt}&
		 \cellcolor{dotfeatures}     & 
		 \cellcolor{dotfeatures}{\color[HTML]{FFFFFF} bottom}  &&& 
		 \cellcolor{dotfeatures} & 
		 \cellcolor{dotfeatures} &
%		 &
%		 \cellcolor{dotfeatures} &
%		 \cellcolor{dotfeatures} & 
%		 \cellcolor{dotfeatures} & 
%		 \cellcolor{dotfeatures} & 
%		 \cellcolor{dotfeatures} & 
%		 \cellcolor{dotfeatures} 
		 \\

		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\cellcolor{fullypdt}& 
		\cellcolor{dotfeatures} & 
		\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} lower bounds} &&& 
		\cellcolor{dotfeatures} & 
		\cellcolor{dotfeatures} & 
		\cellcolor{dotfeatures} 
%		& 
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} & 
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} & 
%		\cellcolor{dotfeatures} & 
%		\cellcolor{dotfeatures} 
		\\

		\cellcolor{dottyfeatures}& 
		\cellcolor{scalafeatures}& 
		\cellcolor{fullypdt}&
		\cellcolor{dotfeatures} & 
		\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} mixins/intersection} &
		\cellcolor{dotfeatures} &
		\cellcolor{dotfeatures} & \cellcolor{dotfeatures} & \cellcolor{dotfeatures} &
%		& 
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures}
		\\
		
		\rowcolor[HTML]{000000} 
		\cellcolor{dottyfeatures}&
		\cellcolor{scalafeatures}&
		\cellcolor{fullypdt}&
		\cellcolor{dotfeatures}& {\color[HTML]{FFFFFF} type members} &
		\cellcolor{dotfeatures}& & & &
		\cellcolor{dotfeatures}
%		&
%		\cellcolor{dotfeatures} &
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}
		\\
		
		\rowcolor[HTML]{000000} 
		\cellcolor{dottyfeatures}&
		\cellcolor{scalafeatures}&
		\cellcolor{fullypdt}&
		\cellcolor{dotfeatures}& {\color[HTML]{FFFFFF} self-names} &
		\cellcolor{dotfeatures}&&&&
		\cellcolor{dotfeatures}
%		&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}&
%		\cellcolor{dotfeatures}
		\\
		
		\rowcolor[HTML]{000000}
		\multirow{-17}{*}{\cellcolor{dottyfeatures}
				\parbox[t]{2mm}{\rotatebox[origin=c]{90}{\makecell{\cellcolor{dottyfeatures}dotty features}}}} & 
		\multirow{-16}{*}{\cellcolor{scalafeatures}\color[HTML]{FFFFFF}
				\parbox[t]{2mm}{\rotatebox[origin=c]{90}{\makecell{\cellcolor{scalafeatures}Scala features}}}} & 
		\multirow{-8}{*}{\cellcolor{fullypdt}\color[HTML]{FFFFFF}
				\parbox[t]{4mm}{\rotatebox[origin=c]{90}{\makecell{\cellcolor{fullypdt}fully path-\\
																									   \cellcolor{fullypdt} dependent types}}}} & 
		\multirow{-7}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF}
				\parbox[t]{0mm}{\rotatebox[origin=c]{90}{DOT}}}} & 
			{\color[HTML]{FFFFFF} upper bounds} & 
			\multirow{-3}{*}{\cellcolor{dotfeatures}} &&&&
			\multirow{-3}{*}{\cellcolor{dotfeatures}} 
%			& 
%			\multirow{-3}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} \checkmark}} &
%			\multirow{-3}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} \checkmark}} & 
%			\multirow{-3}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} \checkmark}} & 
%			\multirow{-3}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} \checkmark}} & 
%			\multirow{-3}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} \checkmark}} &
%			\multirow{-3}{*}{\cellcolor{dotfeatures}{\color[HTML]{FFFFFF} \checkmark}}

	\end{tabular}
\\[1mm]
	\hspace{6.4cm}
	$\uparrow\ $\parbox[t]{20mm}{\textit{paper}\\soundness proof}
	\hspace{4mm}
	$\uparrow\ $\parbox[t]{20mm}{\textit{mechanized}\\soundness proof}
	\caption{Scala calculi that precede DOT}\label{dots}
\end{table}

==> math/precise-typing-new.tex <==
%\begin{definition}[Precise Typing]\label{def-prec}
%  A \emph{typing} derivation is \emph{precise}, denoted as $\typPrecDft t T$, if $\typDft t T$ and the following conditions hold:
%  \begin{enumerate}
%    \item If $t$ is a value, the typing derivation of $t$ ends in \rn{(All-I)} or \tnew{\rn{(\{\}-I!)}}, defined as follows:
%    \newruletrue
%    \infrule[\{\}-I!]
%      {\typdPrec \G x T d T}
%      {\typPrecDft {\tNew x T d} {\tRec x T}}
%    \newrulefalse
%    \item If $t$ is a variable, the typing derivation of $t$ consists only of \rn{(Var)}, \rn{(Rec-E)}, and \rn{(Sub)} steps and every \rn{(Sub)} step makes use of only the subtyping rules \rn{(And$_1-<:$)}, \rn{(And$_2-<:$)}, and \rn{(Trans)}.
%    \item \tnew{If $t=p.a$, $\strong p$, and $\typPrecDft p {\tFldDecStrong a T}$.}
%  \end{enumerate}
%\end{definition}
%\paragraph{Note (Dec-21-2016):} In order for $p.a$ to have the precise type $T$, we need to ensure that if $a$ is assigned to the term $t$ (i.e. $p=...\set{a=t}...$), then $\typPrecDft t T$. To ensure that, we define the strong typing relation for definitions as in (\rn{Def-Path}).


%%\begin{definition}[\tnew{Precise Definition Typing}]\label{def-def-prec}
%  A \emph{definition typing} judgement is \emph{precise} if its 
%  derivation ends in \rn{Def-Trm}, \rn{Def-Typ}, or in one of the following rules:
%
%\newruletrue
%  \infrule[Def-Path!]
%  {\typPrecDft p U \andalso \strong p}
%  {\typdPrecDft {\set{a=p}}{\tFldDecStrong a U}}  

%  \infrule[AndDef-I!]
%  {\typdPrecDft {d_1} {T_1}
%    \andalso
%    \typdPrecDft {d_1} {T_2}
%    \\
%    \dom{d_1},\,\dom{d_2}\text{ disjoint}}
%  {\typdPrecDft {\tAnd {d_1} {d_2}} {\tAnd {T_1} {T_2}}}
%\newrulefalse
%\end{definition}

==> math/tight-subtyping-new.tex <==
\begin{definition}[Tight (Sub)typing]\label{def-tight}
  A typing or subtyping derivation is \emph{tight} in environment $\G$, 
  denoted as
  $\typTightDft t T$ and $\subTightDft T U$,  
  if it only contains the following tight variants of \rn{(Sel$-<:$)} and \rn{($<:-$Sel)} when $\G'=\G$:
  \newruletrue
    \infrule[$<:$-Sel-Tight]
      {\typPrecDft p {\tTypeDec A T T} \andalso 
       \strongTight p}
      {\subTightDft T {p.A}}
    \infrule[Sel-$<:$-Tight]
      {\typPrecDft p {\tTypeDec A T T} \andalso 
       \strongTight p}
      {\subTightDft {p.A} T}
  \newrulefalse
  and the following version of normalization for paths:
  \newruletrue
  \infrule[Norm-Path-\#]
    {\strongTight p \andalso 
     \typTightDft p {\tFldDecStrong a T}}
  {\strongTight {p.a}}
  \newrulefalse
  For environments that extend $\G$, full \rn{(Sel$-<:$)} and \rn{($<:-$Sel)} are permitted.
\end{definition}


==> motivation.tex <==
% \topic{why general paths}
% 
% In the existing DOT calculus, long paths must be expressed in steps:
% for example, the term $x.a.b$ must be deconstructed as
% $\tLet y {x.a} {y.b}$, in which each member selection ($x.a$ and $y.b$) is
% on a variable ($x$ and $y$), not on a general path.
% This decomposition of paths is part of DOT's ANF semantics which ensures that
% before a term is used it is fully evaluated to a variable, which is
% crucial to DOT's type soundness.
% 
% Terms, unlike types, can contain let bindings, which allows terms to refer to all
% the possible paths in a program.
% Types, however, can only reference variables rather than paths, let bindings, or any other terms:
% path-dependent types in DOT are actually \textit{variable}-dependent types.
% As we show in this section, variable-dependent types
% are too restrictive to express the possible type and module dependencies of Scala.
% Specifically, decomposing paths into let bindings prevents us from accessing types that are nested in subpackages
% relative to any of our enclosing packages. \todom{reword this}
% While it is possible in some cases to reorganize the package structure in a program to avoid type-member access into nested packages,
% it is in general impossible to do such a restructuring in the presence of mutually recursive type dependencies.
% 
% \topic{a real-world example}\label{sec:realworld}
% 
% One of the design goals of the Scala language is to enable the
% use of the same language constructs to define both the high-level
% module structure of a program and the details of its implementation.
% More specifically, in Scala, packages and nested subpackages behave much
% like objects, and can be modeled as nested objects in DOT.

Suppose we are implementing the following simplified excerpt from Dotty, the compiler for Scala~3~\cite{dotty}:
\todom{confirm that this corresponds to Dotty}
\begin{lstlisting}[language=Scala,basicstyle=\scalalst]
package root {
    /*\textcolor{gray}{\textbf{package} scala \{...\}}*/
    package dotty {
        package core {
            object Types {
                class Type
                class TypeRef extends Type {
                    val symbol: /*\textbf{core.Symbols.Symbol}*/ = ... }}
            object Symbols {
                class Symbol {
                    val tpe: /*\textbf{core.Types.Type}*/ = ... }}}}}
\end{lstlisting}
\todom{remove the root and scala packages since we don't mention them}
Type references (\code{TypeRef}) are types (\code{Type}) that have an
underlying class or trait definition (\code{Symbol}),
while definitions (\code{Symbol}) in the language also have a type (\code{Type}).
Additionally, \code{TypeRef}s and \code{Symbol}s are declared in different packages,
\code{core.Types} and \code{core.Symbols}.
This program therefore contains mutually recursive types that are nested in different packages.

The DOT formalization introduces a self variable inside each object (and package),
and uses fields to refer to objects nested within it. Therefore, in the formalization
of a path-dependent type such as \code{core.Symbols.Symbol}, \code{core} is represented by
the self variable of the \code{core} package, \code{Symbols} is a field member of that package,
and \code{Symbol} is a type member in the \code{Symbols} object. Thus, the type \code{core.Symbols.Symbol}
is dependent on the \emph{path} \code{core.Symbols}, rather than merely a variable. Although
the \code{Symbols} object does have a self variable, so we could refer to the same type with
the variable-dependent type \code{Symbols.Symbol}, the self variable is in scope only inside
the \code{Symbols} object, so the variable-dependent type cannot be used where we need it
inside \code{core.Types.TypeRef}.

\todoo{Think about some way to distinguish self-variables and fields in the text, maybe with different fonts.}


% We now illustrate that this example is not encodable in DOT.
% 
% The packages that make up this Scala program can be modeled in a DOT-like language as follows.%
% \footnote{For now we will use Scala-like syntax to illustrate the main ideas of encoding
%     this example in DOT. Section~\ref{sec:mrt} presents an actual DOT encoding that is based on this example.}
% \todom{On the one hand, TypeRef extending Type makes the example realistic.
%     On the other hand, it adds a complication that doesn't help the understanding of the example.
%     Also, in Section~\ref{sec:mrt} we don't model the inheritance and make Symbol and Type take
%     constructor parameters}
% \begin{lstlisting}[language=Scala,basicstyle=\scalalst]
% val root = new {
%     /*\textcolor{gray}{\textbf{val} scala = \textbf{new} \{...\}}*/
%     val dotty = new {
%         val core = new { /*\textbf{core}*/ /*$\Rightarrow$*/
%             val Types = new { /*\textbf{this}*/ /*$\Rightarrow$*/
%                 type Type                                                       // class type
%                 def newType(): /*\textbf{this}*/.Type = ...                                  // constructor
%                 type TypeRef = /*\textbf{this}*/.Type /*$\wedge$*/ {val symbol: /*\textbf{core.Symbols.Symbol}*/} // class type
%                 def newTypeRef(): /*\textbf{this}*/.TypeRef = ... }                          // constructor
%             val Symbols = new { /*\textbf{this}*/ /*$\Rightarrow$*/
%                 type Symbol = {val tpe: /*\textbf{core.Types.Type}*/}                       // class type
%                 def newSymbol(): /*\textbf{this}*/.Symbol = ... }}}}                         // constructor 
% \end{lstlisting}
% We define a single \code{root} object representing the root of the package hierarchy. 
% Inside
% the \code{root} object, we define other objects representing top-level packages
% such as the \code{scala} package in the Scala standard library
% and \code{dotty}, the root package of the Scala compiler.
% Nested packages,
% such as \code{dotty.core}, are represented as objects nested within the \code{dotty}
% object. The classes in a package are represented as type member declarations
% and constructor method declarations inside the DOT object that represents the
% package.
% For example, \code{\textbf{class} TypeRef} is represented as a type member 
% \code{\textbf{type} TypeRef}. \code{TypeRef}'s constructor is encoded as a method \code{newTypeRef()}
% that returns an object of type \code{TypeRef}.
% Additionally, we can use DOT's \textit{type intersection} to encode that \code{TypeRef} extends the \code{Type} class.
% \todom{this is beside the point and we should think how to not say it here}
% 
% To encode this example we need path-dependent types of length greater than one, because
% to typecheck \code{TypeRef}'s \code{symbol} field we need access to \code{core.Symbols.Symbol},
% and to typecheck \code{Symbol}'s \code{tpe} field we need access to \code{core.Types.Type}.
% As discussed above, this is currently impossible in DOT.
% 
% \topic{p.A vs. T\#A}
% 
% \topic{p.A = q.A? object identity through variables/paths}
% 

Types that can depend on values are tightly linked with the issue of
object identity. Recall the example of \code{Node} types that depend
on a \code{Graph}. We want the types \code{g1.Node} and \code{g2.Node}
to be considered distinct even though referential transparency would
suggest that because \code{g1} and \code{g2} are both initialized to the
same expression, \code{g1} and \code{g2} should be the same, and therefore
\code{g1.Node} and \code{g2.Node} should be the same. But then it would
not be possible do distinguish the nodes of different graph instances.

On the other hand, notice that the reference \code{g3} is initialized to be
an alias to the same graph instance as \code{g1}. We therefore want \code{g1.Node}
and \code{g3.Node} to be considered the same type. How can the type system
tell the difference between \code{g2.Node} and \code{g3.Node}, so that the
former is considered distinct from \code{g1.Node}, but the latter is considered
the same? Scala uses singleton types for this purpose. In Scala, \code{g3} can be
typed with the singleton type \code{g1.type} which guarantees that it is an alias
for the same object as \code{g1}. The type system treats paths that are provably aliased
(as evidenced by singleton types) as interchangeable, so it considers \code{g1.Node} and
\code{g3.Node} as the same type.
We add singleton types to
pDOT as well for two reasons: first, we found singleton types useful for formalizing
path-dependent types, and second, adding singleton types enables pDOT to model
the singleton types feature of Scala.




% In the DOT calculus by~\citet{wadlerfest}, variables are used to represent object identity. DOT does not allow us to use values directly
% in function application, field selection, or type selection: instead, a value needs to be assigned to a variable,
% and only through the variable can the value be used. Variables in DOT serve thus a similar purpose
% to references in Scala and other object-oriented languages in which objects are identified through their memory locations:
% two objects \code x and \code y that are initialized with two syntactically equal values, for example,
% \begin{lstlisting}[language=Scala,basicstyle=\scalalst]
% val x = new { type A }
% val y = new { type A }
% \end{lstlisting}
% are considered distinct (\code x $\ne$ \code y), and the types \code{x.A} and \code{y.A} are neither equal nor is one a subtype of the other.
% 
% Should variables also represent object identity in \pdot?
% Consider the following example of a hypothetical version of DOT that supports fully path-dependent types:
% 
% \begin{lstlisting}[language=Scala,basicstyle=\scalalst]
% val graph = new { val nodes = new { type Node } }
% val gnodes = graph.nodes
% val node: gnodes.Node
% def addNode(a: graph.nodes.Node): Unit
% addNode(node)  // should this typecheck?
% \end{lstlisting}
% Since \code{gnodes} is instantiated with \code{graph.nodes}, the types \code{graph.nodes.Node}
% and \code{gnodes.Node} should represent the same type,
% and we should be able to pass \code{node} into \code{addNode}.
% However, if we do not treat the path \code{graph.nodes} as the identity of the nested object
% \code{\textbf{new}~\{\textbf{type} Node\}}
% and allow \code{graph.nodes} to reduce to that object, we will lose the information that \code{gnodes} and \code{graph.nodes}
% both lead to the same object, which will raise a type error in the last line.
% 
% \topic{singletons}
% 
% We can use a path-dependent type $x.a.A$ if $x$ is defined to
% be $\tNew x T {\{a=v\}}$, where the value $v$ is a literal object
% that assigns some concrete type $T$ to type member $A$.
% %
% We can use a path-dependent type $x.a.A$ if $x$ is defined to
% be $\tLet y v {\tNew x T {\{a=y\}}}$, where the same value $v$
% is first bound to some variable $y$. More generally, we can further allow
% $y$ to be replaced with an arbitrary path.
% %
% 
% However, in both of these examples, the value $v$ is concrete and explicitly
% specified. There is limited utility in using a path-dependent type to abstract
% over some concrete type when we must explicitly include the concrete type
% with the definition of the abstract type. In their full generality, we wish
% to be able to use path-dependent types as placeholders for unknown types that
% will be supplied later, perhaps when the module that we are defining is
% combined with some other module. More concretely, we wish to use path-dependent
% types defined as follows:
% $
% \tLambda{y}{\tTypeDec{A}{\bot}{\top}}{
%     \tLet x {\tNew x T {\{a=y\}}} t
% }$.
% Here, the path $x.a$ refers to the same object as $y$, so the path-dependent
% type $x.a.A$ is abstract: we know that it is the same type as $y.A$, but we
% do not know which concrete type $x.a.A$ will represent
% until the function is called and some specific concrete type is passed as
% an argument for $y.A$. This power of abstraction is the main motivation
% for having path-dependent types in a language in the first place.
% 
% Our development so far allows this example, so what is the problem?
% \emph{We} know that $x.a.A$ and $y.A$ are the same type, but the
% type system does not: $x.a.A$ is neither a subtype nor a supertype of $y.A$.
% If $y$ were bound to an explicit value $v$ that gave $y.A$ some concrete
% type $T$, we would be able to say that $T <: y.A <: T$ and $T <: x.a.A <: T$,
% and thus conclude that $x.a.A$ is both a subtype and a supertype of $y.A$ by
% transitivity through $T$. But when the concrete type $T$ that will be assigned
% to the abstract type members is not known, when it is kept abstract until
% later, we lose the ability to reason about the relationships between
% path-dependent types. To support abstraction in modules, an expressive
% language must enable reasoning about types even when those types are
% still left abstract. Specifically, DOT should allow us to conclude that
% $x.a.A$ and $y.A$ are equivalent by subtyping even when we do not yet know
% which concrete type they will eventually be bound to. More generally,
% all path-dependent types should be considered to be equivalent if they
% can be traced back to some common type that they were derived from, such
% as $y.A$.
% 
% To support this subtyping between abstract types, we add singleton types.
% \todoo{finish this section}
% 
% \topic{Why formalize general paths (Scala ``overshoots'')}

By formalizing abstract type members and path-dependent types DOT
establishes a theoretical foundation for a variety of programming-language features. In particular, DOT
aims to formalize a module system that contains modules as first-class values and supports abstraction over types as object members.

However, by limiting itself to variable-dependent types DOT can model only special cases of any programming-language features
that depend on path-dependent types. As a result, the DOT calculus not sufficient for formalizing
\todom{rewrite this to be more appreciative of DOT}
\begin{itemize}
    \item a realistic module system, since it must include nested modules and recursive type dependencies;
    \item family polymorphism;
    \item covariant specialization;
    \item classes, traits, and mixin composition in Scala.
\end{itemize}
Therefore, to answer the question of whether Scala's path-dependent types are sound we need a calculus that formalizes them.
In the next section we present an overview of our approach to establishing such a formalization.

%Limiting itself to ANF, in particular to variable-dependent types, is DOT's way to underapproximate Scala's type selections on arbitrary \textit{stable} 
%paths $x.a_1\dots a_n$ which must consist of immutable fields $a_i$.%
%\footnote{Additionally, using \codeft{-strict} mode, the Dotty compiler now includes additional checks on the paths that participate in
%    path-dependent types. To the best of our knowledge, it is not known whether the checks are exhaustive, type-safe,
%    or overly restrictive.}
%Neither Scala nor any realistic programming language restricts itself to ANF.
\todom{Somewhere in the introduction we should say that we will use Wadlerfest DOT and that we denote it as \DOT. Then
we should replace all occurrences of DOT with \DOT.}

\topic{contributions}

